A Note on Antenna Selection in Gaussian MIMO Channels: Capacity Guarantees and Bounds

We consider the problem of selecting $k_t \times k_r$ antennas from a Gaussian MIMO channel with $n_t \times n_r$ antennas, where $k_t \leq n_t$ and $k_r \leq n_r$. We prove the following two results that hold universally, in the sense that they do not depend on the channel coefficients: (i) The capacity of the best $k_t \times k_r$ subchannel is always lower bounded by a fraction $\frac{k_t k_r}{n_t n_r}$ of the full capacity (with $n_t \times n_r$ antennas). This bound is tight as the channel coefficients diminish in magnitude. (ii) There always exists a selection of $k_t \times k_r$ antennas (including the best) that achieves a fraction greater than $\frac{\min(k_t ,k_r)}{\min(n_t,n_r)}$ of the full capacity within an additive constant that is independent of the coefficients in the channel matrix. The key mathematical idea that allows us to derive these universal bounds is to directly relate the determinants of principle sub-matrices of a Hermitian matrix to the determinant of the entire matrix.

==> conclusions.tex <==
\section{Conclusion}

==> illustrations.tex <==
\section{Illustrations}

==> introduction.tex <==
\section{Introduction}

The problem of antenna selection in MIMO channels has been extensively studied in the literature.
Most of the existing works (CITE) have addressed the issue for fading MIMO channels, and proposed (low-complexity) antenna selection algorithms that many-a-time achieve near-optimal scaling performance at high SNR--i.e., they are diversity-multiplexing-tradeoff (DMT) optimal.
However, in these results, the finite SNR performance of antenna selection almost always depends on the channel statistics, and are not universal in nature.
Moreover, to the best of our knowledge, there exists no complete characterization of the fundamental limit of information flow, when a subset of available (transmit and receive) antennas are invoked for communication.

In this paper, we look at the antenna selection problem for an instance of the Gaussian MIMO channel, and derive fundamental bounds on the capacity of the best sub-channel, as a fraction of the capacity of the full MIMO channel.
Our results relate the capacity of the best sub-channel to that of the complete channel using the total number of transmit and receive antennas ($N_t$ and $N_r$), as well as the number of transmit and receive antennas to be selected for communication ($k_t$ and $k_r$):
i.e., the results are not dependent on the channel coefficients in the MIMO matrix.
Also, the results are valid for any instance of the Gaussian MIMO channel, rendering it stronger than a high-SNR DMT-optimal bound.
Any such bound is probabilistic in nature, while our bounds are entirely deterministic.

Ideologically, one can think of these results along the lines of wireless network simplification \cite{simplification_single}, where the authors derive a fundamental limit on the performance of the best subnetwork with $k$ relays, in an $N$-relay diamond network.
This work provides a similar guarantee on the best sub-channel performance for MIMO, albeit the nature of the results and the tools required to obtain them are quite disparate.

To obtain our results, we relate the determinants of principal sub-matrices (matrices with same row and column indices removed) of a Hermitian matrix to that of the entire Hermitian matrix.
This way of approaching the problem allows us to avoid bounding the individual singular values of the MIMO channel matrix, $H$, which often leads to channel-dependent results with regards to selected sub-channel performance.

Specifically, we prove two classes of bounds for MIMO antenna selection in this paper.
First, we show that the best $k_t \times k_r$ sub-channel in the $N_t \times N_r$ MIMO channel achieves at least a fraction $\frac{k_t\cdot k_r}{N_t \cdot N_r}$ of the full channel capacity.
In practice, examples of channels where this bound is tight appear at rather low SNRs: an example being when every coefficient in the MIMO channel matrix are equal, and tend to zero in the limit.
Hence, this bound is useful as a fundamental guarantee on selection capacity when operating at very low SNR regimes (we give examples in Sec. ).
The second, more interesting bound states that the best sub-channel achieves at least a fraction $\frac{\min\{k_t, k_r\}}{\min\{N_t, N_r\}}$ of the full channel capacity, within an additive constant that is independent of the channels.
This bound is more relevant when we move away from the very low SNR regimes, and a sub-channel that achieves this bound, is also DMT optimal, as we argue in Sec. .
An useful way to interpret the second bound is that for every MIMO channel matrix, the best sub-channel achieves the same fraction of the capacity as dictated by the degrees of freedom in the high-SNR DMT characterization, with the approximation guarantee being of a constant-gap type, which is much stronger than the exponential dominance guarantee provided by DMT-type solutions.


==> notations.tex <==
\section{Notations}
For a set containing the elements $\{1,2,3 \dots, n\}$, we represent it with the shorthand $[n]$.

